Average-case Acceleration Through Spectral Density Estimation

We develop a framework for the average-case analysis of random quadratic problems and derive algorithms that are optimal under this analysis. This yields a new class of methods that achieve acceleration given a model of the Hessian's eigenvalue distribution. We develop explicit algorithms for the uniform, Marchenko-Pastur, and exponential distributions. These methods are momentum-based algorithms, whose hyper-parameters can be estimated without knowledge of the Hessian's smallest singular value, in contrast with classical accelerated methods like Nesterov acceleration and Polyak momentum. Through empirical benchmarks on quadratic and logistic regression problems, we identify regimes in which the the proposed methods improve over classical (worst-case) accelerated methods.

==> sections/proofs/estimate_mp_moments.tex <==
\begin{proof}
    Since $\HH \succeq 0$, we have that
    \[
        \|\HH\|_2 = \lambda_{\max}(\HH) \quad \text{and} \quad \frac{tr(\HH)}{d} = \frac{\sum_{i=1}^d \lambda_i(\HH)}{d}.
    \]
    Moreover, the parameters of the Marchenko-Pastur satify
    \[
        \lambda_{\max} = \sigma^2(\sqrt{r}+1)^2 \quad \text{and} \quad \sigma^2r = \mathbb{E}_i[\lambda_i(\HH)].
    \]
    When $d\rightarrow \infty$, we thus have to solve
    \[
        \begin{cases}
            \sigma^2(\sqrt{r}+1)^2 & = \|\HH\|_2 \\
            \sigma^2r & = \frac{tr(\HH)}{d}.
        \end{cases}
    \]
    Taking the root of the first equation, and after removing the second, we have that
    \[
        \sigma = \sqrt{\|\HH\|_2} - \sqrt{\frac{tr(\HH)}{d}}.
    \]
    Then, substituting this value in the second equation gives the desired result.
\end{proof}

==> sections/proofs/estimate_trace_norm.tex <==
\begin{proof}
  The first estimator corresponds to the power method, while the second follows immediately from
  \[
    \tr(\HH) = \frac{1}{\sigma^2}\tr(\HH \sigma^2\textbf{I}) = \frac{1}{\sigma^2}\tr(\HH \mathbb{E}[w^Tw]) = \frac{1}{\sigma^2}\EE\tr(w^T\HH w),
  \]
  if $w$ is a vector with i.i.d. entries, with variance $\sigma^2$.
\end{proof}

==> sections/proofs/optimal_fisher_proof.tex <==
\begin{proof} 
    consider any polynomial $P=P_t$ of degree $t$ such that $P(0) = 1$. Now, consider the residual polynomial $R$ where
    \[
        P(x)-P^*(x) = xR(x), \quad \deg(R) = t-1.
    \]
    The residual polynomial is multiplied by $\xx$ since $0$ is a root of $P(x)-P^{\star}(x)$, since
    \[
        P(0)-P^{\star}(0) = 1-1 = 0.
    \] 
    We now show that if 
    \[
        P^{\star} \text{ is orthogonal w.r.t } \lambda\mu(\lambda) \qquad \text{and} \qquad  P \in \arg\min_P \langle P, P \rangle = \int_{\mathbb
        R}P^2(\lambda)\lambda\mu(\dif \lambda),
    \]
    then $R = 0$, thus implying that $P^{\star} = P$. Indeed,
    \[
        \langle P,P \rangle = \langle P^{\star}, P^{\star} \rangle + \langle \xx R, \xx R \rangle + 2 \langle P^{\star}, \xx R \rangle
    \]
    However,
    \begin{align*}
         \langle P^{\star}, \xx R \rangle & = \int  P^{\star}(\lambda) \lambda R(\lambda) \dif \mu(\lambda)\\
         & = \int  P^{\star}(\lambda)  R(\lambda) \lambda\dif \mu(\lambda)\\
         & = 0
    \end{align*}
    The last equality follows from the fact that the degree of $P^{\star}$ is equal to $t$. This means the polynomial is orthogonal to all other polynomial of degree $t-1$, w.r.t to $\lambda\dif \mu(\lambda)$. Thus,
    \[
        \langle P,P \rangle = \langle P^*, P^* \rangle + \langle \xx R, \xx R \rangle = \underbrace{\|P^{\star}\|^2}_{>0} + \underbrace{\|\xx R\|^2}_{\geq 0}.
    \]
    Since $P$ is the minimal polynomial, $R$ has to be always $0$, which proves the proposition.
\end{proof}
